SPACE: Unsupervised Object-Oriented Scene Representation via Spatial Attention and Decomposition

The ability to decompose complex multi-object scenes into meaningful abstractions like objects is fundamental to achieve higher-level cognition. Previous approaches for unsupervised object-oriented scene representation learning are either based on spatial-attention or scene-mixture approaches and limited in scalability which is a main obstacle towards modeling real-world scenes. In this paper, we propose a generative latent variable model, called SPACE, that provides a unified probabilistic modeling framework that combines the best of spatial-attention and scene-mixture approaches. SPACE can explicitly provide factorized object representations for foreground objects while also decomposing background segments of complex morphology. Previous models are good at either of these, but not both. SPACE also resolves the scalability problems of previous methods by incorporating parallel spatial-attention and thus is applicable to scenes with a large number of objects without performance degradations. We show through experiments on Atari and 3D-Rooms that SPACE achieves the above properties consistently in comparison to SPAIR, IODINE, and GENESIS. Results of our experiments can be found on our project website: https://sites.google.com/view/space-project-page

==> bloss-svp.tex <==
The foreground module is sensitive to the prior of $\rvz^\where$ while modeling objects with varying sizes. If the prior is set to be small, then the model tends to split the larger objects and have multiple bounding boxes on it and when the prior is large, the model does not capture smaller objects in the scene, hence, causing a trade-off between the two priors. In order to palliate this problem we introduce an auxiliary loss which we call the \textit{boundary loss}. In the boundary loss, we construct a boundary of gap $b$ inside each glimpse. So, if the glimpse is of dimensions $\math{gs}\times\math{gs}$ then the size of the boundary would be $gs-b\times gs-b$ and we restrict the object to be inside this boundary and penalize the model if the object's mask goes beyond the boundary. In this way, if the model tries to split the large objects into smaller chunks, the left over region between the boundary and the glimpse is penalized. A detailed implementation of the boundary loss is mentioned in Appendix \ref{ax:aux_loss}.



==> evaluations_svp.tex <==
% Outline:
% - Datasets intro
% - Qualitative 
% Convergence & Speed
% - Quantitative

We evaluate our model on two datasets:

\begin{itemize}
    \item \textbf{Atari} \citep{bellemare13arcade}: For each game, we sample 60,000 random images from a pretrained agent \citep{wu2016tensorpack}. We split the images into 50,000 for the training set, 5,000 for the validation set, and 5,000 for the testing set. Each image is preprocessed into a size of $128\times128$ pixels with BGR color channels. We present the results for the games Space Invaders, Air Raid, River Raid, and Montezuma's Revenge. We also train our model on a dataset of 10 games jointly, where we have 8,000 training images, 1,000 validation images, and 1,000 testing images for each game. A detailed list of Atari games (static and dynamic) used for training has been mentioned in Appendix C.
    \item \textbf{3D Room}: This dataset consists of images of a walled enclosure with a random number of objects on the floor. In order to test the scalability of our model, we use both a Small 3D Room dataset that has 4-8 objects and a Large 3D room dataset that has 18-24 objects. Each image is taken from a random camera angle and the colors of the objects, walls, floor, and sky are also chosen at random.
\end{itemize}

\textbf{Baselines}: We compare our model with the following baselines: IODINE, GENESIS, and SPAIR.
Since SPAIR does not have an explicit background component, we add an additional VAE for processing the background.
The complete details of the architecture used is given in Appendix D.
Additionally, we test against two implementations of SPAIR: one where we train on the entire image using a $16 \times 16$ grid and another where we train on small $4 \times 4$ patches that correspond to $32 \times 32$ pixels.
The latter is consistent with the original SPAIR paper's experiments on Space Invaders and is done because training on the larger grid size is slow due to the sequential nature of the latent inference in SPAIR.

Each of the baseline models has a different decompositional capacity, which we define as the capability of the model to decompose the scene into its semantic constituents such as the foreground and the background.
The foreground further consists of individual objects and the background contains semantically segmented components.
For SPACE, the decompositional capacity is equal to the number of grid cells $H\times W$
(which is the maximum number of foreground objects that can be detected) plus the number of background components $K$.
For SPAIR, the decompositional capacity is equal to the number of grid cells $H \times W$. For IODINE and GENESIS, the decompositional capcity is equal to the number of components $K$.

% YW: not sure if we need to say this. We will call this out as we discuss the qualitative results below.
%We evaluate our model by testing it on images requiring various decompositional capacities ranging from 16 to 256. and found that the model generalizes as well as scales up efficiently whereas, other methods fail to work for decompositional capacities greater than $\sim20$. Thus, our comparison to the baselines is rather limited to low decompositional capacity but for completeness we also evaluate against existing works for higher capacities.

\subsection{Qualitative Comparison of Representations}
Figures \ref{fig:eval:qualitative-3d}, \ref{fig:eval:qualitative-atari}, and \ref{fig:eval:qualitative-montezuma} show sample scene decompositions from our experiments.
Note that SPAIR does not use component masks and IODINE and GENESIS do not separate foreground from background so those cells are left empty.
Additionally, we only display a few representative components for IODINE and GENESIS since we ran those experiments with larger $K$ than can be displayed.
From Figure \ref{fig:eval:qualitative-3d}, we see that SPACE is able to both create bounding boxes for the foreground objects as well as provide a clean segmentation of the background walls, ground, and sky.
We also see that the $16 \times 16$ implementation of SPAIR works well in this environment, although as we will see in section 4.3, it seems to produce multiple overlapping bounding boxes for the same object.
!!TODO:SPAIR 4x4patch!! \yifu{@Skand @Weihao please add this commentary once available}
IODINE also seems to be able to segment the objects and background into separate components.
However, it occasionally does not properly decompose objects (eg. the orange ball in the Small 3D Room experiment is missing from the reconstruction) and may generate blurry objects.
GENESIS, on the other hand, seems to only be able to segment that background and cannot capture the foreground objects into its components.

In Figure \ref{fig:eval:qualitative-atari}, we see that GENESIS and IODINE are not able to detect foreground objects correctly and mostly just segment the more static background. SPACE and SPAIR, on the other hand, are able to detect the foreground objects correctly. 
However, in Space Invaders, the shields near the bottom of the screen are detected as background in the $16 \times 16$ version of SPAIR, whereas SPACE is able to detect them as foreground. The $4 \times 4$ patch version of SPAIR is able to correctly detect the shields as part of the foreground, but it also incorrectly detects the ground on the bottom of the image as multiple foreground objects. This is a limitation of the $4 \times 4$ patch training since the receptive field of each patch is limited so it cannot detect objects bigger than that receptive field. We see a similar problem in Air Raid where many objects are detected as foreground objects. We also see in Air Raid that the $16 \times 16$ version of SPAIR splits objects into two whereas SPACE is able to correctly bound the objects. This may be attributed to our addition of the auxilary boundary loss in the SPACE model. Lastly, we see that SPACE is able to cleanly segment the background in River Raid, where the background dynamically changes. !!TODO: compare this with other results as they come in!! \yifu{@Skand @Weihao}



\textbf{Low Decomposition Capacity} 
In this setting, we compare our model on both on Atari games as well as on 3D Rooms (small) datasets with $<20$ components. For Atari we choose .... games \svp{@Weihao complete this, @Skand...I think for this part we should run exps in low decomposition setting, like using small number of cells and components?(in order to clarify that all baselines work well for low standard:low decomposition)} and for the 3D Rooms we have images consisting of $4\sim8$ objects \svp{@Yi-Fu confirm this range}. The images are of $128\times128$ and all the models are trained on complete images. As expected, SPAIR and SPACE perform very similar in terms of foreground detection, IODINE performs ... and GENESIS... \svp{@Yi-Fu complete this}. Experiments in this setting provide evidence that the baselines were implemented in the right fashion.

\\
\textbf{High Decomposition Capacity} 
In this setting, we train the models to test their decompositional capacity. We train them on Space Invaders Atari game and on 3D Room (large) dataset that consists of $18\sim24$ objects along with complex backgrounds. SPAIR, being sequential (in inferring the latents) scales poorly to higher capacities and thus the authors train the model on small random patches of Space Invaders. Hence, we also train a SPAIR on random patches of $32\times32$ size with $4\times4$ cells, so as to replicate original SPAIR training. Note that, in our experiments, SPAIR worked well for this limited setting as shown in Fig (##) because the background of Space Invaders is simply black, but it failed to model the background in the case of 3D Room dataset. This is primarily because a patch from a complex image cannot provide information about the dynamics of the scene, hence creating a confusion for the model in separating the components.

IODINE and GENESIS analysis \svp{@Yi-Fu complete this}

%% Speed
\subsection{Speed Comparison} 
In this section we compare SPACE with other existing works in the aspect of time taken per iteration and also time taken for the convergence of the model. 

\subsubsection{Iteration Processing Time}
We compare SPACE with 5 components and 1 component against SPAIR, IODINE and GENESIS for varying decompositional capacities. For a fair comparison, we consider two variants of IODINE and GENESIS with the background modeling 5 and 1 components respectively. IODINE, being a fully sequential model that renders each component in one RNN step consumes the maximum time per iteration. This is followed by GENESIS that ... \svp{@Zhixuan - describe why GENESIS takes time briefly} ... Albeit SPAIR does not use any recurrent network, but it does process the cells in a sequential way which makes the inference slow. On the other hand, SPACE employs a parallel processing for the foreground which makes it scalable to be able to showcase a larger decompositional capacity when compared to other aforementioned methods. It is evident from Fig (##) that not only does SPACE consumes less time during inference but also adding additional background components reduces the inference speed by a mere margin.

\subsubsection{Convergence}
It is not sufficient to evaluate SPACE only on the basis of time per iteration. It is also essential to compare the convergence (wall-clock) time so as to assert the scalability of SPACE over other methods. In Fig (##) we compare against other methods for varying decompositional capacities by plotting the mean squared error (MSE) against the wall-clock time. It is evident from the plots that as we increase the capacity of the model, it becomes pragmatically impossible to train IODINE and GENESIS. We also note that it becomes arduous to train on SPAIR for scenes with decompositional capacity of 256, whereas SPACE converges much earlier than other methods hence corroborating the scalability of SPACE to higher capacities.

\subsection{Quantitative Metrics}
Apart from the qualitative and speed comparisons we also compare with SPAIR on object detection metrics such as Average Precision, Accuracy and Error Rate in Table (##). We perform this to show that despite the foreground module being a parallel one, SPACE can still perform very similar to that of SPAIR with enhanced inference as well as training speed. We only evalute the metrics on 3D Room (small and large) since we have the ground truth bounding box associated with each of the objects in the scene.

==> tables/metrics_021320.tex <==
\scalebox{0.7}{
\begin{tabular}{@{}lllllll@{}}
    \toprule
    Model                 & Dataset       & \begin{tabular}[c]{@{}l@{}}Avg. Precision\\ $\text{IoU Threshold}=0.5$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Avg. Precision\\ $\text{IoU Threshold}\in[0.5:0.05:0.95]$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Object Count\\ Error Rate\end{tabular}\\ \midrule
    SPACE ($16\times 16$) & 3D-Room Large & 0.8942  & 0.4608  & 0.0507     \\
    SPACE-WB ($16\times 16$) & 3D-Room Large & 0.8925  & 0.4428  & 0.0947     \\
    SPAIR ($16\times 16$) & 3D-Room Large & 0.9076  & 0.4453 & 0.0427     \\
    \midrule
    SPACE ($8\times 8$)   & 3D-Room Small & 0.9057 & 0.5203 & 0.0330     \\
    SPACE-WB ($8\times 8$)   & 3D-Room Small & 0.9048 & 0.5057 & 0.0566     \\
    SPAIR ($8\times 8$) & 3D-Room Small & 0.9036 & 0.4883 & 0.0257 \\
    \bottomrule
\end{tabular}}

==> tables/metrics_03022020.tex <==
\scalebox{0.7}{
\begin{tabular}{@{}lllllll@{}}
    \toprule
    Model                 & Dataset       & \begin{tabular}[c]{@{}l@{}}Avg. Precision\\ $\text{IoU Threshold}=0.5$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Avg. Precision\\ $\text{IoU Threshold}\in[0.5:0.05:0.95]$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Object Count\\ Error Rate\end{tabular}\\ \midrule
    SPACE ($16\times 16$) & 3D-Room Large & 0.8942  & 0.4608  & 0.0507     \\
    % SPACE ($16\times 16$) & 3D-Room Large & 0.8925  & 0.4428  & 0.0947     \\
    SPAIR ($16\times 16$) & 3D-Room Large & 0.9076  & 0.4453 & 0.0427     \\
    \midrule
    % SPACE ($8\times 8$)   & 3D-Room Small & 0.9057 & 0.5203 & 0.0330     \\
    SPACE ($8\times 8$)   & 3D-Room Small & 0.9048 & 0.5057 & 0.0566     \\
    SPAIR ($8\times 8$) & 3D-Room Small & 0.9036 & 0.4883 & 0.0257 \\
    \bottomrule
\end{tabular}}

==> tables/metrics_old.tex <==
\scalebox{0.7}{
\begin{tabular}{@{}lllllll@{}}
    \toprule
    Model                 & Dataset       & \begin{tabular}[c]{@{}l@{}}Avg. Precision\\ $\text{IoU Threshold}=0.5$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Avg. Precision\\ $\text{IoU Threshold}\in[0.5:0.05:0.95]$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Object Count\\ Error Rate\end{tabular}\\ \midrule
    SPACE ($16\times 16$) & 3D-Room Large & 0.7256                                                                    & 0.2346  & 0.0541     \\
    SPAIR ($16\times 16$) & 3D-Room Large & 0.7131                                                                    & 0.2596 & 0.1279     \\
    \midrule
    SPACE ($8\times 8$)   & 3D-Room Small & 0.6177                                                                    & 0.2091 & 0.0889     \\
    SPAIR ($8\times 8$) & 3D-Room Small & 0.6016 & 0.1718 & 0.2473 \\
    \bottomrule
\end{tabular}}
